Toric structures on near-symplectic 4-manifolds

A near-symplectic structure on a 4-manifold is a closed 2-form that is symplectic away from the 1-dimensional submanifold along which it vanishes and that satisfies a certain transversality condition along this vanishing locus. We investigate near-symplectic 4-manifolds equipped with singular Lagrangian torus fibrations which are locally induced by effective Hamiltonian torus actions. We show how such a structure is completely characterized by a singular integral affine structure on the base of the fibration whenever the vanishing locus is nonempty. The base equipped with this geometric structure generalizes the moment map image of a toric 4-manifold in the spirit of earlier work by the second author on almost toric symplectic 4-manifolds. We use the geometric structure on the base to investigate the problem of making given smooth torus actions on 4-manifolds symplectic or Hamiltonian with respect to near-symplectic structures and to give interesting constructions of structures which are locally given by torus actions but have nontrivial global monodromy.

==> 4Possibilities.tex <==
\font\thinlinefont=cmr5
\mbox{\beginpicture
\setcoordinatesystem units <0.8cm,0.7cm>
\unitlength=1.04987cm
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
\setshadesymbol ({\thinlinefont .})
\setlinear
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdots < 0.0953cm>
{\color[rgb]{0,0,0}\plot  2.857 23.336  3.334 23.812 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  2.857 22.860  3.810 23.812 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  2.857 22.384  4.286 23.812 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  2.857 21.907  4.763 23.812 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  2.857 21.431  5.239 23.812 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  2.857 20.955  5.715 23.812 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  2.857 20.479  3.952 21.573 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  2.857 20.003  3.810 20.955 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  3.334 20.003  3.810 20.479 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  4.227 21.848  5.715 23.336 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  4.568 21.713  5.715 22.860 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  4.703 21.372  5.715 22.384 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  4.763 20.955  5.715 21.907 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  4.763 20.479  5.715 21.431 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  4.763 20.003  5.715 20.955 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.239 20.003  5.715 20.479 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setsolid
{\color[rgb]{0,0,0}\putrule from  2.857 20.003 to  2.857 23.812
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.715 20.003 to  5.715 23.812
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  3.810 20.003 to  3.810 20.009
\putrule from  3.810 20.009 to  3.810 20.024
\putrule from  3.810 20.024 to  3.810 20.049
\plot  3.810 20.049  3.812 20.089 /
\putrule from  3.812 20.089 to  3.812 20.144
\plot  3.812 20.144  3.814 20.212 /
\plot  3.814 20.212  3.816 20.290 /
\plot  3.816 20.290  3.821 20.381 /
\plot  3.821 20.381  3.823 20.477 /
\plot  3.823 20.477  3.827 20.578 /
\plot  3.827 20.578  3.831 20.678 /
\plot  3.831 20.678  3.838 20.777 /
\plot  3.838 20.777  3.844 20.875 /
\plot  3.844 20.875  3.850 20.963 /
\plot  3.850 20.963  3.857 21.050 /
\plot  3.857 21.050  3.863 21.129 /
\plot  3.863 21.129  3.871 21.201 /
\plot  3.871 21.201  3.880 21.266 /
\plot  3.880 21.266  3.890 21.325 /
\plot  3.890 21.325  3.901 21.380 /
\plot  3.901 21.380  3.912 21.431 /
\plot  3.912 21.431  3.924 21.476 /
\plot  3.924 21.476  3.937 21.518 /
\plot  3.937 21.518  3.952 21.556 /
\plot  3.952 21.556  3.969 21.590 /
\plot  3.969 21.590  3.986 21.620 /
\plot  3.986 21.620  4.003 21.647 /
\plot  4.003 21.647  4.020 21.675 /
\plot  4.020 21.675  4.041 21.698 /
\plot  4.041 21.698  4.060 21.721 /
\plot  4.060 21.721  4.083 21.740 /
\plot  4.083 21.740  4.106 21.759 /
\plot  4.106 21.759  4.130 21.774 /
\plot  4.130 21.774  4.153 21.789 /
\plot  4.153 21.789  4.180 21.800 /
\plot  4.180 21.800  4.206 21.808 /
\plot  4.206 21.808  4.231 21.814 /
\plot  4.231 21.814  4.259 21.819 /
\putrule from  4.259 21.819 to  4.286 21.819
\putrule from  4.286 21.819 to  4.314 21.819
\plot  4.314 21.819  4.341 21.814 /
\plot  4.341 21.814  4.367 21.808 /
\plot  4.367 21.808  4.392 21.800 /
\plot  4.392 21.800  4.420 21.789 /
\plot  4.420 21.789  4.443 21.774 /
\plot  4.443 21.774  4.466 21.759 /
\plot  4.466 21.759  4.489 21.740 /
\plot  4.489 21.740  4.513 21.721 /
\plot  4.513 21.721  4.532 21.698 /
\plot  4.532 21.698  4.553 21.675 /
\plot  4.553 21.675  4.570 21.647 /
\plot  4.570 21.647  4.587 21.620 /
\plot  4.587 21.620  4.604 21.590 /
\plot  4.604 21.590  4.621 21.556 /
\plot  4.621 21.556  4.636 21.518 /
\plot  4.636 21.518  4.648 21.476 /
\plot  4.648 21.476  4.661 21.431 /
\plot  4.661 21.431  4.671 21.380 /
\plot  4.671 21.380  4.682 21.325 /
\plot  4.682 21.325  4.693 21.266 /
\plot  4.693 21.266  4.701 21.201 /
\plot  4.701 21.201  4.710 21.129 /
\plot  4.710 21.129  4.716 21.050 /
\plot  4.716 21.050  4.722 20.963 /
\plot  4.722 20.963  4.729 20.875 /
\plot  4.729 20.875  4.735 20.777 /
\plot  4.735 20.777  4.741 20.678 /
\plot  4.741 20.678  4.746 20.578 /
\plot  4.746 20.578  4.750 20.477 /
\plot  4.750 20.477  4.752 20.381 /
\plot  4.752 20.381  4.756 20.290 /
\plot  4.756 20.290  4.758 20.212 /
\plot  4.758 20.212  4.760 20.144 /
\putrule from  4.760 20.144 to  4.760 20.089
\plot  4.760 20.089  4.763 20.049 /
\putrule from  4.763 20.049 to  4.763 20.024
\putrule from  4.763 20.024 to  4.763 20.009
\putrule from  4.763 20.009 to  4.763 20.003
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdots < 0.0953cm>
{\color[rgb]{0,0,0}\plot  6.668 20.479  7.144 20.003 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.668 20.955  7.620 20.003 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.668 21.431  8.096 20.003 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.668 21.907  8.572 20.003 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.668 22.384  9.049 20.003 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.668 22.860  9.525 20.003 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.668 23.336  7.762 22.242 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.668 23.812  7.620 22.860 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  7.144 23.812  7.620 23.336 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.037 21.967  9.525 20.479 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.378 22.102  9.525 20.955 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.513 22.443  9.525 21.431 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.572 22.860  9.525 21.907 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.572 23.336  9.525 22.384 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.572 23.812  9.525 22.860 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  9.049 23.812  9.525 23.336 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setsolid
{\color[rgb]{0,0,0}\putrule from  6.668 23.812 to  6.668 20.003
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  9.525 23.812 to  9.525 20.003
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  7.620 23.812 to  7.620 23.806
\putrule from  7.620 23.806 to  7.620 23.791
\putrule from  7.620 23.791 to  7.620 23.766
\plot  7.620 23.766  7.622 23.726 /
\putrule from  7.622 23.726 to  7.622 23.671
\plot  7.622 23.671  7.624 23.603 /
\plot  7.624 23.603  7.626 23.525 /
\plot  7.626 23.525  7.631 23.434 /
\plot  7.631 23.434  7.633 23.338 /
\plot  7.633 23.338  7.637 23.237 /
\plot  7.637 23.237  7.641 23.137 /
\plot  7.641 23.137  7.648 23.038 /
\plot  7.648 23.038  7.654 22.940 /
\plot  7.654 22.940  7.660 22.852 /
\plot  7.660 22.852  7.667 22.765 /
\plot  7.667 22.765  7.673 22.686 /
\plot  7.673 22.686  7.681 22.614 /
\plot  7.681 22.614  7.690 22.549 /
\plot  7.690 22.549  7.700 22.490 /
\plot  7.700 22.490  7.711 22.435 /
\plot  7.711 22.435  7.722 22.384 /
\plot  7.722 22.384  7.734 22.339 /
\plot  7.734 22.339  7.747 22.297 /
\plot  7.747 22.297  7.762 22.259 /
\plot  7.762 22.259  7.779 22.225 /
\plot  7.779 22.225  7.796 22.195 /
\plot  7.796 22.195  7.813 22.168 /
\plot  7.813 22.168  7.830 22.140 /
\plot  7.830 22.140  7.851 22.117 /
\plot  7.851 22.117  7.870 22.094 /
\plot  7.870 22.094  7.893 22.075 /
\plot  7.893 22.075  7.916 22.056 /
\plot  7.916 22.056  7.940 22.041 /
\plot  7.940 22.041  7.963 22.026 /
\plot  7.963 22.026  7.990 22.015 /
\plot  7.990 22.015  8.016 22.007 /
\plot  8.016 22.007  8.041 22.001 /
\plot  8.041 22.001  8.069 21.996 /
\putrule from  8.069 21.996 to  8.096 21.996
\putrule from  8.096 21.996 to  8.124 21.996
\plot  8.124 21.996  8.151 22.001 /
\plot  8.151 22.001  8.177 22.007 /
\plot  8.177 22.007  8.202 22.015 /
\plot  8.202 22.015  8.230 22.026 /
\plot  8.230 22.026  8.253 22.041 /
\plot  8.253 22.041  8.276 22.056 /
\plot  8.276 22.056  8.299 22.075 /
\plot  8.299 22.075  8.323 22.094 /
\plot  8.323 22.094  8.342 22.117 /
\plot  8.342 22.117  8.363 22.140 /
\plot  8.363 22.140  8.380 22.168 /
\plot  8.380 22.168  8.397 22.195 /
\plot  8.397 22.195  8.414 22.225 /
\plot  8.414 22.225  8.431 22.259 /
\plot  8.431 22.259  8.446 22.297 /
\plot  8.446 22.297  8.458 22.339 /
\plot  8.458 22.339  8.471 22.384 /
\plot  8.471 22.384  8.481 22.435 /
\plot  8.481 22.435  8.492 22.490 /
\plot  8.492 22.490  8.503 22.549 /
\plot  8.503 22.549  8.511 22.614 /
\plot  8.511 22.614  8.520 22.686 /
\plot  8.520 22.686  8.526 22.765 /
\plot  8.526 22.765  8.532 22.852 /
\plot  8.532 22.852  8.539 22.940 /
\plot  8.539 22.940  8.545 23.038 /
\plot  8.545 23.038  8.551 23.137 /
\plot  8.551 23.137  8.556 23.237 /
\plot  8.556 23.237  8.560 23.338 /
\plot  8.560 23.338  8.562 23.434 /
\plot  8.562 23.434  8.566 23.525 /
\plot  8.566 23.525  8.568 23.603 /
\plot  8.568 23.603  8.570 23.671 /
\putrule from  8.570 23.671 to  8.570 23.726
\plot  8.570 23.726  8.572 23.766 /
\putrule from  8.572 23.766 to  8.572 23.791
\putrule from  8.572 23.791 to  8.572 23.806
\putrule from  8.572 23.806 to  8.572 23.812
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdots < 0.0953cm>
{\color[rgb]{0,0,0}\plot 10.478 20.003 12.262 21.787 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 10.499 20.500 12.169 22.170 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 10.526 21.004 12.004 22.481 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 10.575 21.529 11.701 22.655 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 10.674 22.104 11.284 22.714 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 10.954 20.003 12.300 21.349 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 11.430 20.003 12.336 20.908 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 11.906 20.003 12.366 20.462 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setsolid
{\color[rgb]{0,0,0}\putrule from 10.478 20.003 to 10.478 20.009
\putrule from 10.478 20.009 to 10.478 20.019
\putrule from 10.478 20.019 to 10.478 20.043
\plot 10.478 20.043 10.480 20.077 /
\plot 10.480 20.077 10.482 20.123 /
\putrule from 10.482 20.123 to 10.482 20.187
\plot 10.482 20.187 10.486 20.263 /
\plot 10.486 20.263 10.488 20.352 /
\plot 10.488 20.352 10.492 20.451 /
\plot 10.492 20.451 10.497 20.561 /
\plot 10.497 20.561 10.503 20.678 /
\plot 10.503 20.678 10.509 20.798 /
\plot 10.509 20.798 10.516 20.923 /
\plot 10.516 20.923 10.524 21.046 /
\plot 10.524 21.046 10.533 21.167 /
\plot 10.533 21.167 10.541 21.283 /
\plot 10.541 21.283 10.552 21.395 /
\plot 10.552 21.395 10.562 21.501 /
\plot 10.562 21.501 10.573 21.603 /
\plot 10.573 21.603 10.585 21.698 /
\plot 10.585 21.698 10.598 21.785 /
\plot 10.598 21.785 10.613 21.867 /
\plot 10.613 21.867 10.628 21.943 /
\plot 10.628 21.943 10.643 22.015 /
\plot 10.643 22.015 10.662 22.079 /
\plot 10.662 22.079 10.679 22.140 /
\plot 10.679 22.140 10.700 22.195 /
\plot 10.700 22.195 10.721 22.248 /
\plot 10.721 22.248 10.744 22.297 /
\plot 10.744 22.297 10.770 22.341 /
\plot 10.770 22.341 10.795 22.384 /
\plot 10.795 22.384 10.823 22.424 /
\plot 10.823 22.424 10.852 22.460 /
\plot 10.852 22.460 10.884 22.496 /
\plot 10.884 22.496 10.918 22.528 /
\plot 10.918 22.528 10.954 22.559 /
\plot 10.954 22.559 10.990 22.587 /
\plot 10.990 22.587 11.028 22.612 /
\plot 11.028 22.612 11.068 22.636 /
\plot 11.068 22.636 11.110 22.657 /
\plot 11.110 22.657 11.153 22.676 /
\plot 11.153 22.676 11.197 22.691 /
\plot 11.197 22.691 11.242 22.705 /
\plot 11.242 22.705 11.288 22.714 /
\plot 11.288 22.714 11.335 22.722 /
\plot 11.335 22.722 11.383 22.727 /
\plot 11.383 22.727 11.430 22.729 /
\plot 11.430 22.729 11.477 22.727 /
\plot 11.477 22.727 11.525 22.722 /
\plot 11.525 22.722 11.572 22.714 /
\plot 11.572 22.714 11.618 22.705 /
\plot 11.618 22.705 11.663 22.691 /
\plot 11.663 22.691 11.707 22.676 /
\plot 11.707 22.676 11.750 22.657 /
\plot 11.750 22.657 11.792 22.636 /
\plot 11.792 22.636 11.832 22.612 /
\plot 11.832 22.612 11.870 22.587 /
\plot 11.870 22.587 11.906 22.559 /
\plot 11.906 22.559 11.942 22.528 /
\plot 11.942 22.528 11.976 22.496 /
\plot 11.976 22.496 12.008 22.460 /
\plot 12.008 22.460 12.037 22.424 /
\plot 12.037 22.424 12.065 22.384 /
\plot 12.065 22.384 12.090 22.341 /
\plot 12.090 22.341 12.116 22.297 /
\plot 12.116 22.297 12.139 22.248 /
\plot 12.139 22.248 12.160 22.195 /
\plot 12.160 22.195 12.181 22.140 /
\plot 12.181 22.140 12.198 22.079 /
\plot 12.198 22.079 12.217 22.015 /
\plot 12.217 22.015 12.232 21.943 /
\plot 12.232 21.943 12.247 21.867 /
\plot 12.247 21.867 12.262 21.785 /
\plot 12.262 21.785 12.275 21.698 /
\plot 12.275 21.698 12.287 21.603 /
\plot 12.287 21.603 12.298 21.501 /
\plot 12.298 21.501 12.308 21.395 /
\plot 12.308 21.395 12.319 21.283 /
\plot 12.319 21.283 12.327 21.167 /
\plot 12.327 21.167 12.336 21.046 /
\plot 12.336 21.046 12.344 20.923 /
\plot 12.344 20.923 12.351 20.798 /
\plot 12.351 20.798 12.357 20.678 /
\plot 12.357 20.678 12.363 20.561 /
\plot 12.363 20.561 12.368 20.451 /
\plot 12.368 20.451 12.372 20.352 /
\plot 12.372 20.352 12.374 20.263 /
\plot 12.374 20.263 12.378 20.187 /
\putrule from 12.378 20.187 to 12.378 20.123
\plot 12.378 20.123 12.380 20.077 /
\plot 12.380 20.077 12.383 20.043 /
\putrule from 12.383 20.043 to 12.383 20.019
\putrule from 12.383 20.019 to 12.383 20.009
\putrule from 12.383 20.009 to 12.383 20.003
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdots < 0.0953cm>
{\color[rgb]{0,0,0}\plot 13.335 23.812 15.119 22.028 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.356 23.315 15.026 21.645 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.384 22.811 14.861 21.334 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.432 22.286 14.558 21.160 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.532 21.711 14.141 21.101 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.811 23.812 15.157 22.466 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 14.287 23.812 15.193 22.907 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 14.764 23.812 15.223 23.353 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setsolid
{\color[rgb]{0,0,0}\putrule from 13.335 23.812 to 13.335 23.806
\putrule from 13.335 23.806 to 13.335 23.796
\putrule from 13.335 23.796 to 13.335 23.772
\plot 13.335 23.772 13.337 23.738 /
\plot 13.337 23.738 13.339 23.692 /
\putrule from 13.339 23.692 to 13.339 23.628
\plot 13.339 23.628 13.343 23.552 /
\plot 13.343 23.552 13.346 23.463 /
\plot 13.346 23.463 13.350 23.364 /
\plot 13.350 23.364 13.354 23.254 /
\plot 13.354 23.254 13.360 23.137 /
\plot 13.360 23.137 13.367 23.017 /
\plot 13.367 23.017 13.373 22.892 /
\plot 13.373 22.892 13.382 22.769 /
\plot 13.382 22.769 13.390 22.648 /
\plot 13.390 22.648 13.399 22.532 /
\plot 13.399 22.532 13.409 22.420 /
\plot 13.409 22.420 13.420 22.314 /
\plot 13.420 22.314 13.430 22.212 /
\plot 13.430 22.212 13.443 22.117 /
\plot 13.443 22.117 13.456 22.030 /
\plot 13.456 22.030 13.470 21.948 /
\plot 13.470 21.948 13.485 21.872 /
\plot 13.485 21.872 13.500 21.800 /
\plot 13.500 21.800 13.519 21.736 /
\plot 13.519 21.736 13.536 21.675 /
\plot 13.536 21.675 13.557 21.620 /
\plot 13.557 21.620 13.578 21.567 /
\plot 13.578 21.567 13.602 21.518 /
\plot 13.602 21.518 13.627 21.474 /
\plot 13.627 21.474 13.652 21.431 /
\plot 13.652 21.431 13.680 21.391 /
\plot 13.680 21.391 13.710 21.355 /
\plot 13.710 21.355 13.741 21.319 /
\plot 13.741 21.319 13.775 21.287 /
\plot 13.775 21.287 13.811 21.256 /
\plot 13.811 21.256 13.847 21.228 /
\plot 13.847 21.228 13.885 21.203 /
\plot 13.885 21.203 13.926 21.179 /
\plot 13.926 21.179 13.968 21.158 /
\plot 13.968 21.158 14.010 21.139 /
\plot 14.010 21.139 14.055 21.124 /
\plot 14.055 21.124 14.099 21.110 /
\plot 14.099 21.110 14.146 21.101 /
\plot 14.146 21.101 14.192 21.093 /
\plot 14.192 21.093 14.241 21.088 /
\plot 14.241 21.088 14.287 21.086 /
\plot 14.287 21.086 14.334 21.088 /
\plot 14.334 21.088 14.383 21.093 /
\plot 14.383 21.093 14.429 21.101 /
\plot 14.429 21.101 14.476 21.110 /
\plot 14.476 21.110 14.520 21.124 /
\plot 14.520 21.124 14.565 21.139 /
\plot 14.565 21.139 14.607 21.158 /
\plot 14.607 21.158 14.649 21.179 /
\plot 14.649 21.179 14.690 21.203 /
\plot 14.690 21.203 14.728 21.228 /
\plot 14.728 21.228 14.764 21.256 /
\plot 14.764 21.256 14.800 21.287 /
\plot 14.800 21.287 14.834 21.319 /
\plot 14.834 21.319 14.865 21.355 /
\plot 14.865 21.355 14.895 21.391 /
\plot 14.895 21.391 14.922 21.431 /
\plot 14.922 21.431 14.948 21.474 /
\plot 14.948 21.474 14.973 21.518 /
\plot 14.973 21.518 14.997 21.567 /
\plot 14.997 21.567 15.018 21.620 /
\plot 15.018 21.620 15.039 21.675 /
\plot 15.039 21.675 15.056 21.736 /
\plot 15.056 21.736 15.075 21.800 /
\plot 15.075 21.800 15.090 21.872 /
\plot 15.090 21.872 15.105 21.948 /
\plot 15.105 21.948 15.119 22.030 /
\plot 15.119 22.030 15.132 22.117 /
\plot 15.132 22.117 15.145 22.212 /
\plot 15.145 22.212 15.155 22.314 /
\plot 15.155 22.314 15.166 22.420 /
\plot 15.166 22.420 15.177 22.532 /
\plot 15.177 22.532 15.185 22.648 /
\plot 15.185 22.648 15.193 22.769 /
\plot 15.193 22.769 15.202 22.892 /
\plot 15.202 22.892 15.208 23.017 /
\plot 15.208 23.017 15.215 23.137 /
\plot 15.215 23.137 15.221 23.254 /
\plot 15.221 23.254 15.225 23.364 /
\plot 15.225 23.364 15.229 23.463 /
\plot 15.229 23.463 15.232 23.552 /
\plot 15.232 23.552 15.236 23.628 /
\putrule from 15.236 23.628 to 15.236 23.692
\plot 15.236 23.692 15.238 23.738 /
\plot 15.238 23.738 15.240 23.772 /
\putrule from 15.240 23.772 to 15.240 23.796
\putrule from 15.240 23.796 to 15.240 23.806
\putrule from 15.240 23.806 to 15.240 23.812
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdots < 0.0953cm>
{\color[rgb]{0,0,0}\plot  1.905 23.812 16.192 23.812 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  1.905 20.003 16.192 20.003 /
}%
\linethickness=0pt
\putrectangle corners at  1.880 23.838 and 16.218 19.977
\endpicture}


==> PeriodicPath.tex <==
\font\thinlinefont=cmr5
\mbox{\beginpicture
\small
\setcoordinatesystem units <0.5cm,0.5cm>
\unitlength=1.00000cm
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
\setshadesymbol ({\thinlinefont .})
\setlinear
%
% Fig ELLIPSE
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\ellipticalarc axes ratio  0.064:0.064  360 degrees 
	from 15.953 17.774 center at 15.890 17.774
}%
%
% Fig ELLIPSE
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\ellipticalarc axes ratio  0.064:0.064  360 degrees 
	from 18.047 16.919 center at 17.983 16.919
}%
%
% Fig ELLIPSE
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\ellipticalarc axes ratio  0.064:0.064  360 degrees 
	from 23.647 19.744 center at 23.584 19.744
}%
%
% Fig ELLIPSE
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\ellipticalarc axes ratio  0.064:0.064  360 degrees 
	from 25.726 18.868 center at 25.662 18.868
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdots < 0.0953cm>
{\color[rgb]{0,0,0}\plot 13.350 12.700 12.080 12.700 /
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
\setsolid
{\color[rgb]{0,0,0}\putrule from 13.282 12.700 to 15.840 12.700
\putrule from 15.822 12.700 to 15.822 17.780
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from 15.947 17.782 to 15.947 17.147
\plot 15.947 17.147 16.804 16.163 /
\plot 16.804 16.163 17.947 16.957 /
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\plot 18.036 16.863 17.549 16.525 /
\plot 17.549 16.525 18.288 15.331 /
\plot 18.288 15.331 19.622 14.633 /
\putrule from 19.622 14.633 to 21.177 14.633
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from 20.991 14.633 to 23.549 14.633
\putrule from 23.531 14.633 to 23.531 19.713
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from 23.641 19.753 to 23.641 19.118
\plot 23.641 19.118 24.498 18.133 /
\plot 24.498 18.133 25.641 18.927 /
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\plot 25.696 18.821 25.210 18.483 /
\plot 25.210 18.483 25.948 17.289 /
\plot 25.948 17.289 27.282 16.590 /
\putrule from 27.282 16.590 to 28.837 16.590
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdots < 0.0953cm>
{\color[rgb]{0,0,0}\plot 28.710 16.586 29.972 16.586 /
}%
\linethickness=0pt
\putrectangle corners at 12.054 19.837 and 29.997 12.653
\endpicture}

